Tabling as a Library with Delimited Control

Tabling is probably the most widely studied extension of Prolog. But despite its importance and practicality, tabling is not implemented by most Prolog systems. Existing approaches require substantial changes to the Prolog engine, which is an investment out of reach of most systems. To enable more widespread adoption, we present a new implementation of tabling in under 600 lines of Prolog code. Our lightweight approach relies on delimited control and provides reasonable performance.

==> memoisation.tex <==
% \documentclass{article}
% \begin{document}
Apart from the termination properties of tabling, the technique can also offer a significant performance gain through memoisation.
Table~\ref{fibo-no-tabling} shows the average execution times for calculating the $n$-th Fibonacci number using standard SLD-resolution.
Contrast these numbers with Table~\ref{fibo-tabling} that shows the average execution time using our tabling implementation (version on branch ``batched-worklist'').


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Benoit: for a nice GRAPH, see my R script in the repository.
% However, this takes more space than the two tables.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Benoit:
% I tried using the subfig package: the tables appeared below each other even after a lot of fiddling.
% I also tried the subcaption package, which is not compatible with the documentclass.
% I hate doing this kind of stuff in LaTeX...
\begin{table}
\begin{minipage}{0.45\linewidth}
{ \footnotesize
\begin{tabular}{*{6}{l}}
$\mathbf{n}$  & 25 & 30  & 35   & 40    & 45 \\
\textbf{Time} & 19 & 210 & 1753 & 16267 & 177725 \\
\end{tabular}
\caption{Average execution times for calculating the $n$-th Fibonacci number using standard SLD-resolution (ms).\label{fibo-no-tabling}}
} % end footnotesize
\end{minipage}
\enskip % Smaller than quad
\begin{minipage}{0.45\linewidth}
{ \footnotesize
\begin{tabular}{*{5}{l}}
$\mathbf{n}$  & 200 & 500 & 750 & 1000 \\
\textbf{Time} & 15  & 69  & 118 & 272  \\
\end{tabular}
\caption{Average execution times for calculating the $n$-th Fibonacci number using our tabling implementation (ms).\label{fibo-tabling}}
} % end footnotesize
\end{minipage}
\end{table}
% \end{document}
% Measurements on the bean server, average out of five runs, branch batched-worklist, date: 02/04/2015.
% 25fib-no-tabling 19
% 30fib-no-tabling 210
% 35fib-no-tabling 1753
% 40fib-no-tabling 16267
% 45fib-no-tabling 177725
% 200fib 15
% 500fib 69
% 750fib 118
% 1000fib 272

% As Marko would like to see these numbers in a graph instead of a silly table, he asked me to prepare this data in a CSV format:
% See file memoisation-data.csv
% Format:
% fibonacci-number-n,execution-time-no-tabling,execution-time-tabling
% question marks indicate the absence of measurement data.
% 25,19,?
% 30,210,?
% 35,1753,?
% 40,16267,?
% 45,177725,?
% 200,?,15
% 500,?,69
% 750,?,118
% 1000,?,272

